Mirage Models Confront the LHC: II. Flux-Stabilized Type IIB String Theory

We continue the study of a class of string-motivated effective supergravity theories in light of current data from the CERN Large Hadron Collider (LHC). In this installment we consider Type IIB string theory compactified on a Calabi-Yau orientifold in the presence of fluxes, in the manner originally formulated by Kachru, et al. We allow for a variety of potential uplift mechanisms and embeddings of the Standard Model field content into D3 and D7 brane configurations. We find that an uplift sector independent of the Kahler moduli, as is the case with anti-D3 branes, is inconsistent with data unless the matter and Higgs sectors are localized on D7 branes exclusively, or are confined to twisted sectors between D3 and D7 branes. We identify regions of parameter space for all possible D-brane configurations that remain consistent with PLANCK observations on the dark matter relic density and measurements of the CP-even Higgs mass at the LHC. Constraints arising from LHC searches at 8 TeV center-of-mass energies, and the LUX dark matter detection experiment, are discussed. The discovery prospects for the remaining parameter space at dark matter direct detection experiments are described, and signatures for detection of superpartners at the LHC, with center-of-mass energy of 14 TeV, are analyzed.

==> Final Draft/basic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% Command definitions %
%%%%%%%%%%%%%%%%%%%%%%%

% This defines a small-caps format for use in math mode (equations)
\DeclareMathAlphabet   {\mathsc}{OT1}{cmr}{m}{sc}

% Define new formatting functions
\newcommand{\nochapter}[1]{
  \chapter*{#1}
  \markboth{#1}{#1}
  \addcontentsline{toc}{chapter}{#1}}
\newcommand{\nnn}{ \nonumber \\ }
%\newcommand{\eqref}[1]{~(\ref{#1})}
\newcommand{\sgspace}{\def\baselinestretch{1.0}}
\newcommand{\dbspace}{\def\baselinestretch{1.8}}
% Left and right formatting
\def\[{\left [}
\def\]{\right ]}
\def\({\left (}
\def\){\right )}
\newcommand{\lang}{\left\langle}
\newcommand{\rang}{\right\rangle}
\newcommand{\lbr}{\left\{}
\newcommand{\rbr}{\right\}}
% Barred quantities
\newcommand{\oline}[1]{\overline{#1}}
\newcommand{\jbar}{\bar{\jmath}}
\newcommand{\ibar}{\bar{\imath}}
% Tildes
\newcommand{\td}[1]{\tilde{#1}}
\newcommand{\wtd}[1]{\widetilde{#1}}
% Caligraphy
\newcommand{\Lag}{\mathcal{L}}
\newcommand{\D}{\mathcal{D}}
% Hatted quantities
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\h}[1]{\hat{#1}}
% Slashed quantities
\newcommand{\notd}{\not{\hspace{-.05in}\pp}}
\newcommand{\notD}{\not{\hspace{-.05in}D}}
\newcommand{\notcD}{\not{\hspace{-.05in}\D}}
% Useful HEP definitions
%\newcommand{\pCL}      {\%~\mathrm{C.L.}}
\newcommand{\MeV}      {~\mathrm{MeV}}
\newcommand{\GeV}      {~\mathrm{GeV}}
\newcommand{\TeV}      {~\mathrm{TeV}}
\newcommand{\MS}       {\mathsc{\overline{MS}}}
\newcommand{\SM}       {\mathsc{sm}}
\newcommand{\EW}       {\mathsc{ew}}
\newcommand{\IR}       {\mathsc{ir}}
\newcommand{\EM}       {\mathsc{em}}
\newcommand{\CP}       {\mathsc{cp}}
\newcommand{\KE}       {\mathsc{ke}}
\newcommand{\VY}       {\mathsc{vy}}
\newcommand{\UV}       {\mathsc{uv}}
\newcommand{\GS}       {\mathsc{gs}}
\newcommand{\PL}       {\mathsc{pl}}
\newcommand{\PV}       {\mathsc{pv}}
\newcommand{\GUT}      {\mathsc{gut}}
\newcommand{\STR}      {\mathsc{str}}
\newcommand{\SUSY}     {\mathsc{susy}}
\newcommand{\MSSM}     {\mathsc{mssm}}
\newcommand{\COND}     {\mathsc{cond}}
\newcommand{\Mpl}{M_{\PL}}
% Supergravity quantities
\newcommand{\superint}{\int\diff^{4}\theta}
\newcommand{\chiral}{\(\bar{\D}^2 - 8R\)}
\newcommand{\achiral}{\({\D}^2 - 8\oline{R}\)}
\newcommand{\Mgrav}{M_{3/2}}
\newcommand{\rpart}[1]{{#1}+\oline{#1}}
\newcommand{\ww}{W^\alpha W_\alpha}
\newcommand{\bww}{\overline{W}_{\dot\alpha} \overline{W}^{\dot\alpha}}
\newcommand{\WaWa}{ W_a^{\alpha} W_{b}^{\alpha}}
\newcommand{\WbWb}{ W^a_{\dot{\alpha}}W^{b\dot{\alpha}}}
\newcommand{\DaDa}{{\D}^{\alpha}{\D}_{\alpha}}
\newcommand{\DbDb}{{\D}_{\dot{\alpha}}{\D}^{\dot{\alpha}}}
\newcommand{\Da}{{\D}_{\alpha}}
\newcommand{\Db}{{\D}^{\dot{\beta}}}
\newcommand{\Dc}{{\D}^{\alpha}}
\newcommand{\Dd}{{\D}_{\dot{\beta}}}
\newcommand{\Wa}{W_{\alpha}}
\newcommand{\Wb}{W^{\dot{\beta}}}
\newcommand{\Wc}{W^{\alpha}}
\newcommand{\Wd}{W_{\dot{\beta}}}
\newcommand{\lowest}{|_{\theta =\bar{\theta}=0}}
\newcommand{\blowest}{\bigg|_{\theta =\bar{\theta}=0}}
% This last one is lowest component without any thetas
\def\Eisen{G_{2}\(t,\bar{t}\)}
\def\bli{\bigg|}
% Put alpha superscript/subscripts
\newcommand{\supal}[1]{{#1}^{\alpha}}
\newcommand{\subal}[1]{{#1}_{\alpha}}
\newcommand{\supdal}[1]{{#1}^{\dot{\alpha}}}
\newcommand{\subdal}[1]{{#1}_{\dot{\alpha}}}
% BGW model quantities
\newcommand{\baal}{b_{a}^{\alpha}}
\newcommand{\baaleff}{\(\baal\)_{\rm eff}}
\newcommand{\bpaleff}{\(b_{+}^{\alpha}\)_{\rm eff}}
\newcommand{\caleff}{\({c_{\alpha}}\)_{\rm eff}}
% Useful shortcuts in formulae
\newcommand{\lhs}      {\mbox{l.h.s.}}
\newcommand{\rhs}      {\mbox{r.h.s.}}
\newcommand{\hc}       {\mathrm{\; h.c. \;}}
\newcommand{\cc}       {\mathrm{\; c.c. \;}}
\newcommand{\pp}{\partial}
\newcommand{\Br}{{\rm Br}}
\newcommand{\Det}{{\rm Det}}
\newcommand{\STr}{{\rm STr}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\btr}{{\bf Tr}}
\newcommand{\diff}{\mbox{d}}
\newcommand{\order}{\mathcal{O}}
\newcommand{\re}{{\rm Re}}
\newcommand{\im}{{\rm Im}}
\newcommand{\lsimeq}{{\stackrel{<}{\sim}}}
\newcommand{\gsimeq}{{\stackrel{>}{\sim}}}
%\newcommand{\loop}{{1\over16\pi^2}}
\newcommand{\loopp}{{1\over32\pi^2}}
\newcommand{\gappeq}{\mathrel{\rlap {\raise.5ex\hbox{$>$}}
{\lower.5ex\hbox{$\sim$}}}}
\newcommand{\lappeq}{\mathrel{\rlap{\raise.5ex\hbox{$<$}}
{\lower.5ex\hbox{$\sim$}}}}
\newcommand{\up}{^{(0)}}
\newcommand{\upp}{^{(1)}}

% Hyphenation list
\hyphenation{su-per-sym-me-try su-per-sym-met-ric sca-lar sca-lars
  coun-ter-term fer-mi-on fer-mi-ons gau-gi-no gau-gi-nos chi-ral
  su-per-mul-ti-plet su-per-po-ten-tial a-no-ma-ly su-per-gra-vi-ty
  non-u-ni-ver-sal non-u-ni-ver-sal-i-ties non-van-ish-ing tri-lin-ear
  bi-lin-ear La-gran-gi-ans coun-ter-terms mul-ti-plet mul-ti-plets
  spur-i-on spur-i-ons non-per-tur-ba-tive grav-i-ti-no per-turb-a-tive
  bi-fun-da-ment-al}

